Fair Set Cover

The potential harms of algorithmic decisions have ignited algorithmic fairness as a central topic in computer science. One of the fundamental problems in computer science is Set Cover, which has numerous applications with societal impacts, such as assembling a small team of individuals that collectively satisfy a range of expertise requirements. However, despite its broad application spectrum and significant potential impact, set cover has yet to be studied through the lens of fairness. Therefore, in this paper, we introduce Fair Set Cover, which aims not only to cover with a minimum-size set but also to satisfy demographic parity in its selection of sets. To this end, we develop multiple versions of fair set cover, study their hardness, and devise efficient approximation algorithms for each variant. Notably, under certain assumptions, our algorithms always guarantee zero-unfairness, with only a small increase in the approximation ratio compared to regular set cover. Furthermore, our experiments on various data sets and across different settings confirm the negligible price of fairness, as (a) the output size increases only slightly (if any) and (b) the time to compute the output does not significantly increase.

==> content/setMultiCover.tex <==
\section{Set Multicover}
\mohsen{Needs more thinking, currently $k O(\log n)$-approx}
In this problem, each $\element_j \in \Elements$ is also associated with a number $r_j$.

{\bf Set Multicover}: Find a minimum sized cover $\cover \subset \Sets$ such that each point $\element_j \in \Elements$ is covered by at least $r_j$ sets.

{\bf Weighted Set Multicover}: Find a cover $\cover \subset \Sets$ with minimum sum of weights (call $w_j$ as the weight of $\set_j \in \Sets$), such that each point $\element_j \in \Elements$ is covered at by at least $r_j$ sets.

Note: In both above definitions, I am allowed to pick {\bf at most one} instance of each set $S_j \in \mathcal{S}$ (aka Contrained Set Multicover).


\subsection{Fair Set Multicover}
Fair Set Multicover ensures that the final cover $\cover$ has an equal number of sets belonging to each color.

\subsubsection{Greedy Algorithm}
Start from an empty set $\cover_1$. In each iteration $i$, add a new pair $(\set_{a, i}, \set_{b, i})$ to $\cover_{i}$ such that $\set_{a, i} \in c_1$ and $\set_{b, i} \in c_2$. Continue this until $X_i$ is your final cover.

Call a point $\element_j \in \Elements$ \emph{alive} if this point is covered by less than $r_j$ sets so far. Let $Y_i$ denote the set of all \emph{alive} points at the iteration $i$ (before executing this iteration). 

In each iteration, pick the pair $(\set_{a, i}, \set_{b, i})$, covering the most \emph{alive} points from $Y_i$ and remove all covered points from $Y_i$ to create $Y_{i + 1}$. For each \emph{alive} point $\element_j$ in $S_a \cup S_b$, assign a price $Price(e_j, q) = \frac{2}{|Y_i \cap (\set_{a, i} \cup \set_{b, i})|}$, where this picked pair is the $q$th pair covering this point since the beginning of algorithm (for more than two colors, use $k$ instead of 2).

% \begin{lemma}
% $\sum_{\element_j \in \Elements} \sum_{q \leq R(e_j)} Price(\element_j, q) = |\cover|$, where $\cover$ is the final collected cover. Where $R(e_j)$ is the number of pairs in $\cover$ that cover $e_j$. Note that $R(e_j)$ might be bigger than $r_j$, because we are picking pairs and $e_j$ might lie in the intersection.
% \end{lemma}


% \begin{proof}
% Each set pair $(\set_{a, i}, \set_{b, i})$ covers $|Y_i \cap (\set_{a, i} \cup S_{b, i})|$ points with price $\frac{2}{|Y_i \cap (S_{a, i} \cup S_{b, i})|}$. As a result, the sum of these values is counting the number of sets in $\cover$.
% \end{proof}

{\bf Theorem 1}: Greedy algorithm gives an $\ln{n}$-approximation ratio. In other words $|\cover| \leq O(\log n) |\optCover|$.

\subsubsection{Proof by Dual Fitting [New Version!]}
The following would be the LP formulation of the Fair Set Multicover. $l$ is a given constant that denotes the number of sets from each color in $\cover$.

Assign a variable $z_t$ for each set $\set_t \in \Sets$ and $\mu = |\Sets|$


\begin{align}
    \min \sum_{1 \leq t \leq \mu} z_t &\\
    &\sum_{t: e_j \in S_t} z_t \geq r_j, \quad \forall j: \element_j \in \Elements\\
    & -z_t \geq -1, \quad \forall 1 \leq t \leq \mu\\
    &\sum_{t: c(S_t) = h} z_t = l, \quad \forall h \in \mathcal{C}
\end{align}

The following is an equivalent LP containing only $\geq$ constraints:

\begin{align}
    \min \sum_{1 \leq t \leq \mu} z_t &\\
    &\sum_{t: e_j \in S_t} z_t \geq r_j, \quad \forall j: \element_j \in \Elements\\
    & -z_t \geq -1, \quad \forall 1 \leq t \leq \mu\\
    &\sum_{t: c(S_t) = h} z_t \geq l, \quad \forall h \in \mathcal{C}\\
    &-\sum_{t: c(S_t) = h} z_t \geq -l, \quad \forall h \in \mathcal{C}
\end{align}

Assign a variable $y_j$ for each $\element_j \in \Elements$ and a new variable $x_t$ for each $\set_t \in \Sets$ and assign two variables $c^+_h$ and $c^-_h$ for each color $h \in \mathcal{C}$. This would be the dual LP:

\begin{align}
    &\max \sum_{1 \leq j \leq n} r_j y_j - \sum_{1 \leq t \leq \mu} x_t + l \sum_{1 \leq h \leq k} c^+_h - l \sum_{1 \leq h \leq k} c^-_h\\
    & \sum_{j: \element_j \in \set_t} y_j - x_t + c^+_{c(S_t)} - c^-_{c(S_t)} \leq 1, \quad \forall t: \set_t \in \Sets
\end{align}

Define $X_{paired}$ as the set of pairs we packed while constructing $\cover$.


For each set $S_t$ in the final cover $\cover$ and each pair $pr \in \cover_{paired}$, define the following functions: 
\begin{itemize}
    \item $g(S_t)$ denotes the number associated with the pair that contains $S_t$.
    \item $p(S_t)$ denotes the pair that picked at iteration $g(S_t)$ (the pair that contains $S_t$). 
    \item $f(S_t)$ denotes the {\bf set} of \emph{alive} points covered by $S_t$ after picking this set in some pair. If an \emph{alive} point lies in the intersection of the two sets in the picked pair $(S_a, S_b)$, this point is only present in one of $f(S_a)$ or $f(S_b)$. WLOG assume the set with the smaller color value $h$, has this point as its \emph{alive} points.
    \item $d(pr, \element_j)$ denotes the number of times $e_j$ has been covered so far, {\bf after} picking the pair $pr$. Note that $\element_j$ should be in either of sets of $pr$.
\end{itemize}

For example, if $(S_a, S_b)$ is the $i$th picked pair, then $g(S_a) = g(S_b) = i$ and also $f(S_a)$ is the set of \emph{alive} points covered at iteration $i$ by $S_a$. The \emph{alive} points in the intersection of $S_a$ and $S_b$ are only present in $f(S_a)$ and not in $f(S_b)$. If $e_j \in S_a$ has been picked $\alpha$ times before iteration $i$, then $d(S_a, e_j) = \alpha + 1$.

Let $c^+_h = c^-_h$ for each $h \in \mathcal{C}$. For each $t$, if $S_t$ is not present in the final cover $\cover$, then assign $x_t = 0$, otherwise assign the following value:

\begin{align}
    x_t = \sum_{j: \element_j \in f(S_t)} (y_j - Price(e_j, d(p(S_t), e_j)))
\end{align}

Define $obj$ to be the objective function of the dual LP which we want to maximize. 

\begin{lemma}
    $obj \geq |\cover|$
\end{lemma}

\begin{proof}
\begin{align}
    obj &= \sum_{1 \leq j \leq n} r_j y_j - \sum_{1 \leq t \leq \mu} x_t + l \sum_{1 \leq h \leq k} c^+_h - l \sum_{1 \leq h \leq k} c^-_h \\
    &= \sum_{1 \leq j \leq n} r_j y_j - \sum_{1 \leq t \leq \mu} x_t\\
    &= \sum_{t: S_t \in \cover} \sum_{e_j: e_j \in f(S_t)} Price(e_j, d(p(S_t), e_j))\\
    &= \sum_{(S_a, S_b) \in X_{paired}} (\sum_{e_j \in S_a} Price(e_j, d((S_a, S_b), e_j)) \\
    &+ \sum_{e_j \in S_b} Price(e_j, d((S_a, S_b), e_j)))\\
    &= \sum_{(S_a, S_b) \in X_{paired}} (|f(S_a)| + |f(S_b)|) \frac{2}{|f(S_a) \cup f(S_b)|}\\
    &= \sum_{(S_a, S_b) \in X_{paired}} 2\\
    &= 2 |X_{paired}| = |X|
\end{align}
    
In the above all the $r_j y_j$ are cancelled out because we have the following fact:

\begin{align}
    f(S_a) \cap f(S_b) = \emptyset, \quad \forall (S_a, S_b) \in X_{paired}
\end{align}


\end{proof}

Now for each variable $y_j$ assign the following value:

\begin{align}
    y_j = Price(e_j, R(e_j))
\end{align}

$R(e_j)$ denotes the number of pairs in $X$ that covered the point $e_j$ when it was \emph{alive}. In other words, $Price(e_j, R(e_j))$ is the last price value assigned to a point $e_j$ in the greedy algorithm (there is no $Price(e_j, x)$ such that $x > R(e_j)$).

Let $S_t \notin \cover$ and $S_t = \{e_{t_\beta}, e_{t_{\beta - 1}}, ..., e_{t_1}\}$. Assume these points are {\bf completely} covered\footnote{They are not alive anymore.} in the given order. For example, $e_{t_i}$ is completely covered before or at the same time as $e_{t_{i - 1}}$ and so on. Define $iter(q)$ to be the iteration in which $e_{t_q}$ is completely covered by some picked pair $(S_{a}, S_{b})$ in the algorithm. There are $q$ alive points in $S_t$ in the iteration $iter(q)$. Let $Y_{iter(q)}$ denote the set of all alive points in $\Elements$ at iteration $iter(q)$. Based on the greedy step in our algorithm, $|Y_{iter(q)} \cap (S_a \cup S_b)| \geq |Y_{iter(q)} \cap S_t|$:

\begin{align}
    Price(e_{t_q}, R(e_{t_q})) &= \frac{2}{|Y_{iter(q)} \cap (S_a \cup S_b)|}\\
    &= \frac{2}{|f(S_a) \cup f(S_b)|}\\
    &\leq \frac{2}{Y_{iter(q)} \cap S_t}\\
    &\leq \frac{2}{q}
\end{align}

{\bf observation 1}: For each $S_t \notin \cover$, $\sum_{e_j \in S_t} Price(e_j, R(e_j)) \leq 2 H_n$. Where $H_n$ is the sum of harmonic series. 

Let $S_d \in \cover$ be one of the picked sets. Define $S_d = \{e_{d_\alpha}, e_{d_{\alpha - 1}, ..., e_1}\}$ the same as before according to the order of completely covering the points of this set. For a value $0 \leq \gamma \leq \alpha$, all the points $C = \{e_{d_\alpha}, e_{d_{\alpha - 1}, ..., e_{d_{\gamma + 1}}}\}$ were completely covered before picking $S_d$, but others were not.

For a $q > \gamma$ let $iter(q)$ be the iteration in which the point $e_{d_{q}}$ has been completely covered by the picked pair $(S_a, S_b)$. Again like before, we can conclude that $Price(e_{d_q}, R(e_{d_q})) \leq \frac{2}{q}$.

Let $S^{\prime}_d$ be the set that is picked alongside $S_d$ in a pair at some point in our algorithm. We have:

\begin{align}
    \sum_{e_j \in f(S_d)} Price(e_j, d(p(S_d), e_j)) &= \sum_{e_j \in f(S_d)} \frac{2}{|f(S_d) \cup f(S^{\prime}_d)|}\\
    &\leq \sum_{e_j \in f(S_d)} \frac{2}{|f(S_d)|}\\
    &= 2
\end{align}


{\bf Observation 2}: 
\begin{align}
    \sum_{e_j \in C_1} Price(e_j, R(e_j)) + \sum_{e_j \in S_d \setminus C_1} Price(e_j, d(p(S_d), e_j)) \leq 2 H_n
\end{align}

Observations 1 and 2 say that for these variable assignments, the constraint in the dual LP does not hold. However, by assigning new variables $x^{\prime}_t = \frac{x_t}{2 H_n}$ and $y^{\prime}_j = \frac{y_j}{2 H_n}$, we would have a feasible solution for the dual LP. Let $opt$ be the optimum solution to primal LP. The objective function of the dual LP would be equal to $\frac{obj}{2 H_n}$:

\begin{align}
    \frac{|X|}{2 H_n} \leq \frac{obj}{2 H_n} \leq opt \leq |X^*|
\end{align}

As a result, $|X| \leq k O(\log n) |X^*|$. Where $k$ is the number of colors.

\subsubsection{Picking Pairs Efficiently}
In the above greedy algorithm, we picked a $k$-tuple at each iteration in $O(n^k)$ time. We can covert this tuple selection to an instance of Fair Max-K-Cover and solve it with an approximation ration of $\frac{e}{e - 1}$ like before Fair Set Cover section.

% \subsection{Fair Weighted Set Multicover}
